Fast Sequence-Based Embedding with Diffusion Graphs

A graph embedding is a representation of graph vertices in a low-dimensional space, which approximately preserves properties such as distances between nodes. Vertex sequence-based embedding procedures use features extracted from linear sequences of nodes to create embeddings using a neural network. In this paper, we propose diffusion graphs as a method to rapidly generate vertex sequences for network embedding. Its computational efficiency is superior to previous methods due to simpler sequence generation, and it produces more accurate results. In experiments, we found that the performance relative to other methods improves with increasing edge density in the graph. In a community detection task, clustering nodes in the embedding space produces better results compared to other sequence-based embedding methods.

==> figures/misses.tex <==
\begin{figure}[h!]
\centering
\captionsetup[subfloat]{width=140pt}

	\begin{tikzpicture}[transform shape]
	\SetVertexNormal[Shape      = circle,
	MinSize    =20pt,
	]
	\Vertex[L=$a$,x=0,y=-1]{1}
	\Vertex[L=$b$,x=1.5,y=-2.5]{2}
	\Vertex[L=$c$,x=1.5,y=0.5]{3}
	
	\tikzstyle{VertexStyle} = []
	\Vertex[L=$$,x=0,y=1]{0}	
\tikzstyle{VertexStyle} = [shape = rectangle]
	
	\tikzstyle{EdgeStyle}=[]
	\Edge[label=$\frac{1}{2}$](1)(2)
	\Edge[label=$\frac{1}{2}$](1)(3)
\end{tikzpicture}

\captionsetup{width=1\textwidth}
\caption[Deriving the sequence generation probabilities]{Example undirected graph with sample sequences and exact sequence sampling probabilities. The graph $\mathcal{G}(V,E)$ is defined by vertex set $V=\{a,b,c,d\}$ and edge set $E=\{(a,b),(a,c),(c,b),(b,d),(c,d)\}$. The sequences have length 3 and all of them originates from vertex $a$. Sequence sampling probabilities show that diffusion trees are biased towards clustered neighbourhoods with short average path lengths.}\label{graph_sample_example_2}
\end{figure}

==> figures/visualizations/barabasi_1/deep_walk_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_1/diffusion_ETT_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_1/diffusion_endpoint_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_1/node2vec_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_2/deep_walk_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_2/deep_walk_3d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]
    \Vertex[L=$$,x=8.58,y=5.34]{0}
    \Vertex[L=$$,x=7.14,y=7.11]{1}
    \Vertex[L=$$,x=7.605,y=6.225]{2}
    \Vertex[L=$$,x=8.325,y=4.065]{3}
    \Vertex[L=$$,x=3.84,y=5.01]{4}
    \Vertex[L=$$,x=6.885,y=7.005]{5}
    \Vertex[L=$$,x=10.125,y=5.52]{6}
    \Vertex[L=$$,x=8.805,y=3.135]{7}
    \Vertex[L=$$,x=10.86,y=5.67]{8}
    \Vertex[L=$$,x=12.675,y=3.93]{9}
    \Vertex[L=$$,x=10.695,y=5.985]{10}
    \Vertex[L=$$,x=8.805,y=4.665]{11}
    \Vertex[L=$$,x=10.26,y=7.53]{12}
    \Vertex[L=$$,x=9.84,y=4.935]{13}
    \Vertex[L=$$,x=6.39,y=7.005]{14}
    \Vertex[L=$$,x=9.84,y=6.54]{15}
    \Vertex[L=$$,x=2.67,y=9.465]{16}
    \Vertex[L=$$,x=3.765,y=8.175]{17}
    \Vertex[L=$$,x=9.99,y=6.645]{18}
    \Vertex[L=$$,x=5.58,y=5.475]{19}
    \Vertex[L=$$,x=8.595,y=3.87]{20}
    \Vertex[L=$$,x=1.5,y=6.885]{21}
    \Vertex[L=$$,x=6.375,y=3.99]{22}
    \Vertex[L=$$,x=9.42,y=5.55]{23}
    \Vertex[L=$$,x=7.95,y=6.585]{24}
    \Vertex[L=$$,x=9.93,y=3.42]{25}
    \Vertex[L=$$,x=7.26,y=1.89]{26}
    \Vertex[L=$$,x=13.305,y=4.68]{27}
    \Vertex[L=$$,x=8.67,y=8.175]{28}
    \Vertex[L=$$,x=8.61,y=3.825]{29}
    \Vertex[L=$$,x=10.98,y=8.025]{30}
    \Vertex[L=$$,x=8.325,y=5.25]{31}
    \Vertex[L=$$,x=7.785,y=9.51]{32}
    \Vertex[L=$$,x=8.775,y=6.285]{33}
    \Vertex[L=$$,x=8.745,y=5.61]{34}
    \Vertex[L=$$,x=7.26,y=5.04]{35}
    \Vertex[L=$$,x=5.265,y=1.935]{36}
    \Vertex[L=$$,x=7.41,y=4.335]{37}
    \Vertex[L=$$,x=5.43,y=6.105]{38}
    \Vertex[L=$$,x=12.285,y=6.705]{39}
    \Vertex[L=$$,x=4.095,y=8.55]{40}
    \Vertex[L=$$,x=7.605,y=1.71]{41}
    \Vertex[L=$$,x=8.265,y=4.62]{42}
    \Vertex[L=$$,x=7.65,y=5.79]{43}
    \Vertex[L=$$,x=2.97,y=9.525]{44}
    \Vertex[L=$$,x=8.895,y=11.43]{45}
    \Vertex[L=$$,x=11.13,y=8.4]{46}
    \Vertex[L=$$,x=10.185,y=6.555]{47}
    \Vertex[L=$$,x=4.8,y=7.92]{48}
    \Vertex[L=$$,x=10.86,y=6.03]{49}
    \Vertex[L=$$,x=7.425,y=9.255]{50}
    \Vertex[L=$$,x=9.24,y=7.785]{51}
    \Vertex[L=$$,x=8.685,y=6.03]{52}
    \Vertex[L=$$,x=1.35,y=5.79]{53}
    \Vertex[L=$$,x=14.055,y=5.82]{54}
    \Vertex[L=$$,x=8.415,y=2.445]{55}
    \Vertex[L=$$,x=3.33,y=1.425]{56}
    \Vertex[L=$$,x=11.55,y=5.295]{57}
    \Vertex[L=$$,x=3.225,y=3.195]{58}
    \Vertex[L=$$,x=6.645,y=2.94]{59}
    \Vertex[L=$$,x=8.565,y=3.435]{60}
    \Vertex[L=$$,x=6.615,y=5.1]{61}
    \Vertex[L=$$,x=8.22,y=2.775]{62}
    \Vertex[L=$$,x=11.355,y=6.93]{63}
    \Vertex[L=$$,x=7.62,y=6.075]{64}
    \Vertex[L=$$,x=5.505,y=1.965]{65}
    \Vertex[L=$$,x=9.315,y=5.16]{66}
    \Vertex[L=$$,x=6.33,y=13.095]{67}
    \Vertex[L=$$,x=8.37,y=4.815]{68}
    \Vertex[L=$$,x=13.005,y=3.69]{69}
    \Vertex[L=$$,x=13.485,y=8.79]{70}
    \Vertex[L=$$,x=5.25,y=7.965]{71}
    \Vertex[L=$$,x=8.91,y=5.52]{72}
    \Vertex[L=$$,x=9.465,y=5.25]{73}
    \Vertex[L=$$,x=2.085,y=0.105]{74}
    \Vertex[L=$$,x=11.22,y=2.01]{75}
    \Vertex[L=$$,x=9.975,y=6.03]{76}
    \Vertex[L=$$,x=10.575,y=7.305]{77}
    \Vertex[L=$$,x=8.715,y=3.435]{78}
    \Vertex[L=$$,x=1.665,y=4.56]{79}
    \Vertex[L=$$,x=10.65,y=10.935]{80}
    \Vertex[L=$$,x=8.025,y=6.09]{81}
    \Vertex[L=$$,x=11.955,y=3.465]{82}
    \Vertex[L=$$,x=5.04,y=3.105]{83}
    \Vertex[L=$$,x=8.52,y=5.79]{84}
    \Vertex[L=$$,x=5.115,y=5.43]{85}
    \Vertex[L=$$,x=12.825,y=2.595]{86}
    \Vertex[L=$$,x=2.295,y=7.29]{87}
    \Vertex[L=$$,x=13.785,y=4.86]{88}
    \Vertex[L=$$,x=5.655,y=4.155]{89}
    \Vertex[L=$$,x=6.825,y=3.915]{90}
    \Vertex[L=$$,x=7.95,y=6.15]{91}
    \Vertex[L=$$,x=7.17,y=8.88]{92}
    \Vertex[L=$$,x=8.625,y=7.245]{93}
    \Vertex[L=$$,x=9.24,y=4.065]{94}
    \Vertex[L=$$,x=1.605,y=4.065]{95}
    \Vertex[L=$$,x=8.82,y=5.76]{96}
    \Vertex[L=$$,x=0.09,y=5.79]{97}
    \Vertex[L=$$,x=9.93,y=7.26]{98}
    \Vertex[L=$$,x=9.27,y=15.0]{99}
    \Vertex[L=$$,x=13.125,y=8.88]{100}
    \Vertex[L=$$,x=11.76,y=9.675]{101}
    \Vertex[L=$$,x=2.7,y=13.14]{102}
    \Vertex[L=$$,x=6.27,y=2.07]{103}
    \Vertex[L=$$,x=9.63,y=3.66]{104}
    \Vertex[L=$$,x=5.325,y=3.96]{105}
    \Vertex[L=$$,x=11.28,y=13.92]{106}
    \Vertex[L=$$,x=13.245,y=2.235]{107}
    \Vertex[L=$$,x=3.6,y=10.08]{108}
    \Vertex[L=$$,x=12.675,y=7.965]{109}
    \Vertex[L=$$,x=8.46,y=5.28]{110}
    \Vertex[L=$$,x=11.025,y=3.195]{111}
    \Vertex[L=$$,x=11.22,y=7.08]{112}
    \Vertex[L=$$,x=6.525,y=2.025]{113}
    \Vertex[L=$$,x=11.475,y=9.24]{114}
    \Vertex[L=$$,x=6.105,y=11.115]{115}
    \Vertex[L=$$,x=0.885,y=3.345]{116}
    \Vertex[L=$$,x=4.68,y=9.045]{117}
    \Vertex[L=$$,x=5.7,y=5.985]{118}
    \Vertex[L=$$,x=7.65,y=7.23]{119}
    \Vertex[L=$$,x=6.51,y=4.395]{120}
    \Vertex[L=$$,x=9.66,y=7.23]{121}
    \Vertex[L=$$,x=11.25,y=3.39]{122}
    \Vertex[L=$$,x=0.645,y=14.445]{123}
    \Vertex[L=$$,x=8.145,y=1.53]{124}
    \Vertex[L=$$,x=9.195,y=0.0]{125}
    \Vertex[L=$$,x=15.0,y=9.51]{126}
    \Vertex[L=$$,x=14.055,y=2.925]{127}
    \Vertex[L=$$,x=9.99,y=0.915]{128}
    \Vertex[L=$$,x=10.86,y=11.085]{129}
    \Vertex[L=$$,x=9.075,y=1.425]{130}
    \Vertex[L=$$,x=10.56,y=3.915]{131}
    \Vertex[L=$$,x=0.0,y=8.82]{132}
    \Vertex[L=$$,x=8.52,y=7.26]{133}
    \Vertex[L=$$,x=8.265,y=2.175]{134}
    \Vertex[L=$$,x=7.275,y=5.145]{135}
    \Vertex[L=$$,x=13.875,y=9.915]{136}
    \Vertex[L=$$,x=12.705,y=3.6]{137}
    \Vertex[L=$$,x=1.11,y=4.23]{138}
    \Vertex[L=$$,x=3.555,y=7.35]{139}
    \Vertex[L=$$,x=4.44,y=7.74]{140}
    \Vertex[L=$$,x=8.73,y=4.8]{141}
    \Vertex[L=$$,x=4.785,y=4.125]{142}
    \Vertex[L=$$,x=9.795,y=5.55]{143}
    \Vertex[L=$$,x=9.9,y=8.445]{144}
    \Vertex[L=$$,x=9.375,y=1.47]{145}
    \Vertex[L=$$,x=10.875,y=4.59]{146}
    \Vertex[L=$$,x=12.81,y=4.815]{147}
    \Vertex[L=$$,x=7.71,y=14.97]{148}
    \Vertex[L=$$,x=13.905,y=5.82]{149}
\AddVertexColor{gray!90, draw=black}{0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26,27,28,29,30,31,32,33,34,35,36,37,38,39,40,41,42,43,44,45,46,47,48,49,50,51,52,53,54,55,56,57,58,59,60,61,62,63,64,65,66,67,68,69,70,71,72,73,74,75,76,77,78,79,80,81,82,83,84,85,86,87,88,89,90,91,92,93,94,95,96,97,98,99,100,101,102,103,104,105,106,107,108,109,110,111,112,113,114,115,116,117,118,119,120,121,122,123,124,125,126,127,128,129,130,131,132,133,134,135,136,137,138,139,140,141,142,143,144,145,146,147,148,149}
\tikzstyle{EdgeStyle}=[line width=0.7pt, opacity = 0.3]
\tikzstyle{LabelStyle}=[fill=white]
    \Edge[label=](0)(2)
    \Edge[label=](0)(3)
    \Edge[label=](0)(7)
    \Edge[label=](0)(8)
    \Edge[label=](0)(9)
    \Edge[label=](0)(12)
    \Edge[label=](0)(13)
    \Edge[label=](0)(14)
    \Edge[label=](0)(17)
    \Edge[label=](0)(18)
    \Edge[label=](0)(23)
    \Edge[label=](0)(25)
    \Edge[label=](0)(31)
    \Edge[label=](0)(33)
    \Edge[label=](0)(36)
    \Edge[label=](0)(37)
    \Edge[label=](0)(64)
    \Edge[label=](0)(68)
    \Edge[label=](0)(75)
    \Edge[label=](0)(81)
    \Edge[label=](0)(82)
    \Edge[label=](0)(89)
    \Edge[label=](0)(95)
    \Edge[label=](0)(96)
    \Edge[label=](0)(98)
    \Edge[label=](0)(101)
    \Edge[label=](0)(108)
    \Edge[label=](1)(33)
    \Edge[label=](1)(2)
    \Edge[label=](1)(4)
    \Edge[label=](1)(5)
    \Edge[label=](1)(38)
    \Edge[label=](1)(15)
    \Edge[label=](1)(50)
    \Edge[label=](1)(52)
    \Edge[label=](1)(117)
    \Edge[label=](1)(118)
    \Edge[label=](1)(121)
    \Edge[label=](2)(3)
    \Edge[label=](2)(4)
    \Edge[label=](2)(5)
    \Edge[label=](2)(6)
    \Edge[label=](2)(135)
    \Edge[label=](2)(12)
    \Edge[label=](2)(16)
    \Edge[label=](2)(19)
    \Edge[label=](2)(21)
    \Edge[label=](2)(28)
    \Edge[label=](2)(34)
    \Edge[label=](2)(42)
    \Edge[label=](2)(48)
    \Edge[label=](2)(49)
    \Edge[label=](2)(51)
    \Edge[label=](2)(61)
    \Edge[label=](2)(72)
    \Edge[label=](2)(73)
    \Edge[label=](2)(91)
    \Edge[label=](2)(92)
    \Edge[label=](3)(36)
    \Edge[label=](3)(134)
    \Edge[label=](3)(7)
    \Edge[label=](3)(122)
    \Edge[label=](3)(11)
    \Edge[label=](3)(13)
    \Edge[label=](3)(66)
    \Edge[label=](3)(24)
    \Edge[label=](3)(68)
    \Edge[label=](3)(26)
    \Edge[label=](3)(29)
    \Edge[label=](3)(62)
    \Edge[label=](4)(118)
    \Edge[label=](4)(38)
    \Edge[label=](4)(138)
    \Edge[label=](4)(142)
    \Edge[label=](4)(79)
    \Edge[label=](4)(50)
    \Edge[label=](4)(19)
    \Edge[label=](4)(21)
    \Edge[label=](4)(22)
    \Edge[label=](4)(58)
    \Edge[label=](4)(59)
    \Edge[label=](4)(85)
    \Edge[label=](4)(53)
    \Edge[label=](5)(133)
    \Edge[label=](5)(6)
    \Edge[label=](5)(71)
    \Edge[label=](5)(139)
    \Edge[label=](5)(77)
    \Edge[label=](5)(87)
    \Edge[label=](5)(24)
    \Edge[label=](6)(70)
    \Edge[label=](6)(8)
    \Edge[label=](6)(9)
    \Edge[label=](6)(55)
    \Edge[label=](6)(141)
    \Edge[label=](6)(110)
    \Edge[label=](6)(15)
    \Edge[label=](6)(20)
    \Edge[label=](6)(23)
    \Edge[label=](6)(57)
    \Edge[label=](6)(47)
    \Edge[label=](7)(128)
    \Edge[label=](7)(130)
    \Edge[label=](7)(10)
    \Edge[label=](7)(145)
    \Edge[label=](7)(22)
    \Edge[label=](7)(25)
    \Edge[label=](7)(27)
    \Edge[label=](7)(37)
    \Edge[label=](7)(41)
    \Edge[label=](7)(42)
    \Edge[label=](7)(63)
    \Edge[label=](7)(65)
    \Edge[label=](7)(78)
    \Edge[label=](7)(90)
    \Edge[label=](7)(94)
    \Edge[label=](7)(103)
    \Edge[label=](7)(104)
    \Edge[label=](7)(111)
    \Edge[label=](7)(113)
    \Edge[label=](7)(124)
    \Edge[label=](8)(73)
    \Edge[label=](8)(10)
    \Edge[label=](8)(11)
    \Edge[label=](8)(76)
    \Edge[label=](8)(77)
    \Edge[label=](8)(146)
    \Edge[label=](8)(147)
    \Edge[label=](8)(63)
    \Edge[label=](9)(111)
    \Edge[label=](9)(147)
    \Edge[label=](9)(86)
    \Edge[label=](9)(127)
    \Edge[label=](10)(39)
    \Edge[label=](10)(109)
    \Edge[label=](10)(14)
    \Edge[label=](10)(112)
    \Edge[label=](10)(84)
    \Edge[label=](10)(27)
    \Edge[label=](11)(43)
    \Edge[label=](11)(60)
    \Edge[label=](12)(35)
    \Edge[label=](12)(133)
    \Edge[label=](12)(109)
    \Edge[label=](12)(45)
    \Edge[label=](12)(46)
    \Edge[label=](12)(47)
    \Edge[label=](12)(49)
    \Edge[label=](12)(114)
    \Edge[label=](12)(143)
    \Edge[label=](12)(28)
    \Edge[label=](12)(30)
    \Edge[label=](13)(34)
    \Edge[label=](13)(69)
    \Edge[label=](13)(72)
    \Edge[label=](13)(18)
    \Edge[label=](13)(20)
    \Edge[label=](14)(32)
    \Edge[label=](14)(35)
    \Edge[label=](14)(40)
    \Edge[label=](14)(64)
    \Edge[label=](14)(43)
    \Edge[label=](14)(44)
    \Edge[label=](14)(16)
    \Edge[label=](14)(140)
    \Edge[label=](14)(85)
    \Edge[label=](15)(66)
    \Edge[label=](15)(39)
    \Edge[label=](15)(51)
    \Edge[label=](15)(30)
    \Edge[label=](15)(31)
    \Edge[label=](16)(132)
    \Edge[label=](16)(102)
    \Edge[label=](16)(40)
    \Edge[label=](16)(44)
    \Edge[label=](16)(17)
    \Edge[label=](17)(48)
    \Edge[label=](17)(119)
    \Edge[label=](17)(140)
    \Edge[label=](17)(87)
    \Edge[label=](18)(70)
    \Edge[label=](18)(119)
    \Edge[label=](20)(104)
    \Edge[label=](20)(105)
    \Edge[label=](20)(75)
    \Edge[label=](20)(78)
    \Edge[label=](20)(143)
    \Edge[label=](20)(120)
    \Edge[label=](20)(29)
    \Edge[label=](21)(132)
    \Edge[label=](21)(139)
    \Edge[label=](21)(53)
    \Edge[label=](24)(115)
    \Edge[label=](25)(137)
    \Edge[label=](25)(26)
    \Edge[label=](26)(56)
    \Edge[label=](26)(55)
    \Edge[label=](26)(41)
    \Edge[label=](27)(69)
    \Edge[label=](27)(149)
    \Edge[label=](27)(54)
    \Edge[label=](27)(88)
    \Edge[label=](28)(32)
    \Edge[label=](30)(46)
    \Edge[label=](31)(90)
    \Edge[label=](32)(45)
    \Edge[label=](33)(76)
    \Edge[label=](35)(56)
    \Edge[label=](36)(65)
    \Edge[label=](36)(74)
    \Edge[label=](36)(113)
    \Edge[label=](37)(89)
    \Edge[label=](37)(135)
    \Edge[label=](37)(141)
    \Edge[label=](39)(144)
    \Edge[label=](39)(112)
    \Edge[label=](39)(52)
    \Edge[label=](39)(149)
    \Edge[label=](39)(54)
    \Edge[label=](39)(57)
    \Edge[label=](44)(108)
    \Edge[label=](45)(129)
    \Edge[label=](45)(67)
    \Edge[label=](48)(71)
    \Edge[label=](49)(88)
    \Edge[label=](50)(99)
    \Edge[label=](50)(148)
    \Edge[label=](50)(67)
    \Edge[label=](51)(80)
    \Edge[label=](51)(93)
    \Edge[label=](52)(96)
    \Edge[label=](52)(61)
    \Edge[label=](55)(131)
    \Edge[label=](55)(60)
    \Edge[label=](55)(59)
    \Edge[label=](55)(124)
    \Edge[label=](55)(62)
    \Edge[label=](56)(74)
    \Edge[label=](56)(58)
    \Edge[label=](56)(103)
    \Edge[label=](57)(131)
    \Edge[label=](59)(125)
    \Edge[label=](61)(110)
    \Edge[label=](61)(79)
    \Edge[label=](61)(81)
    \Edge[label=](61)(83)
    \Edge[label=](61)(84)
    \Edge[label=](63)(80)
    \Edge[label=](63)(136)
    \Edge[label=](63)(129)
    \Edge[label=](65)(83)
    \Edge[label=](67)(102)
    \Edge[label=](67)(144)
    \Edge[label=](67)(115)
    \Edge[label=](67)(92)
    \Edge[label=](69)(107)
    \Edge[label=](69)(122)
    \Edge[label=](70)(100)
    \Edge[label=](70)(101)
    \Edge[label=](70)(136)
    \Edge[label=](70)(126)
    \Edge[label=](73)(94)
    \Edge[label=](75)(128)
    \Edge[label=](75)(107)
    \Edge[label=](75)(82)
    \Edge[label=](75)(86)
    \Edge[label=](75)(125)
    \Edge[label=](77)(100)
    \Edge[label=](79)(97)
    \Edge[label=](79)(105)
    \Edge[label=](79)(95)
    \Edge[label=](80)(99)
    \Edge[label=](80)(98)
    \Edge[label=](81)(93)
    \Edge[label=](82)(127)
    \Edge[label=](84)(91)
    \Edge[label=](85)(120)
    \Edge[label=](87)(97)
    \Edge[label=](88)(137)
    \Edge[label=](89)(116)
    \Edge[label=](90)(142)
    \Edge[label=](95)(138)
    \Edge[label=](95)(116)
    \Edge[label=](99)(148)
    \Edge[label=](99)(106)
    \Edge[label=](101)(106)
    \Edge[label=](101)(114)
    \Edge[label=](102)(123)
    \Edge[label=](104)(146)
    \Edge[label=](108)(123)
    \Edge[label=](108)(117)
    \Edge[label=](109)(126)
    \Edge[label=](112)(121)
    \Edge[label=](124)(134)
    \Edge[label=](125)(130)
    \Edge[label=](128)(145)
\end{tikzpicture}
\label{dg}
\caption{Example Title}
\end{figure}


==> figures/visualizations/barabasi_2/diffusion_ETT_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_2/diffusion_ETT_3d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]
    \Vertex[L=$$,x=10.59,y=5.01]{0}
    \Vertex[L=$$,x=10.185,y=6.585]{1}
    \Vertex[L=$$,x=10.125,y=5.835]{2}
    \Vertex[L=$$,x=8.97,y=3.585]{3}
    \Vertex[L=$$,x=5.955,y=6.33]{4}
    \Vertex[L=$$,x=9.87,y=6.9]{5}
    \Vertex[L=$$,x=10.875,y=4.665]{6}
    \Vertex[L=$$,x=7.965,y=3.06]{7}
    \Vertex[L=$$,x=11.88,y=4.83]{8}
    \Vertex[L=$$,x=11.235,y=2.49]{9}
    \Vertex[L=$$,x=11.52,y=4.965]{10}
    \Vertex[L=$$,x=9.96,y=4.05]{11}
    \Vertex[L=$$,x=12.18,y=6.015]{12}
    \Vertex[L=$$,x=10.74,y=4.38]{13}
    \Vertex[L=$$,x=9.33,y=7.83]{14}
    \Vertex[L=$$,x=11.37,y=5.4]{15}
    \Vertex[L=$$,x=7.425,y=11.055]{16}
    \Vertex[L=$$,x=7.14,y=9.57]{17}
    \Vertex[L=$$,x=11.475,y=5.835]{18}
    \Vertex[L=$$,x=7.965,y=6.315]{19}
    \Vertex[L=$$,x=9.825,y=4.32]{20}
    \Vertex[L=$$,x=4.875,y=9.135]{21}
    \Vertex[L=$$,x=7.755,y=4.575]{22}
    \Vertex[L=$$,x=10.68,y=4.95]{23}
    \Vertex[L=$$,x=10.77,y=6.585]{24}
    \Vertex[L=$$,x=7.935,y=2.16]{25}
    \Vertex[L=$$,x=4.95,y=1.545]{26}
    \Vertex[L=$$,x=11.325,y=3.03]{27}
    \Vertex[L=$$,x=11.31,y=6.87]{28}
    \Vertex[L=$$,x=8.865,y=3.72]{29}
    \Vertex[L=$$,x=12.765,y=5.895]{30}
    \Vertex[L=$$,x=9.675,y=4.935]{31}
    \Vertex[L=$$,x=11.1,y=8.52]{32}
    \Vertex[L=$$,x=10.995,y=5.76]{33}
    \Vertex[L=$$,x=10.59,y=5.145]{34}
    \Vertex[L=$$,x=9.975,y=5.07]{35}
    \Vertex[L=$$,x=4.35,y=3.03]{36}
    \Vertex[L=$$,x=6.3,y=4.71]{37}
    \Vertex[L=$$,x=8.43,y=6.645]{38}
    \Vertex[L=$$,x=11.985,y=4.56]{39}
    \Vertex[L=$$,x=7.98,y=10.14]{40}
    \Vertex[L=$$,x=5.115,y=1.56]{41}
    \Vertex[L=$$,x=9.6,y=4.635]{42}
    \Vertex[L=$$,x=10.215,y=5.46]{43}
    \Vertex[L=$$,x=7.5,y=11.955]{44}
    \Vertex[L=$$,x=12.135,y=9.51]{45}
    \Vertex[L=$$,x=13.215,y=6.27]{46}
    \Vertex[L=$$,x=11.835,y=5.34]{47}
    \Vertex[L=$$,x=7.605,y=9.09]{48}
    \Vertex[L=$$,x=11.49,y=4.44]{49}
    \Vertex[L=$$,x=11.295,y=8.16]{50}
    \Vertex[L=$$,x=11.64,y=7.335]{51}
    \Vertex[L=$$,x=10.545,y=5.295]{52}
    \Vertex[L=$$,x=3.885,y=8.685]{53}
    \Vertex[L=$$,x=12.345,y=3.72]{54}
    \Vertex[L=$$,x=5.895,y=0.96]{55}
    \Vertex[L=$$,x=2.19,y=2.61]{56}
    \Vertex[L=$$,x=10.47,y=3.6]{57}
    \Vertex[L=$$,x=4.755,y=4.71]{58}
    \Vertex[L=$$,x=8.625,y=3.495]{59}
    \Vertex[L=$$,x=8.01,y=2.535]{60}
    \Vertex[L=$$,x=8.76,y=5.385]{61}
    \Vertex[L=$$,x=6.585,y=1.59]{62}
    \Vertex[L=$$,x=13.41,y=8.31]{63}
    \Vertex[L=$$,x=9.735,y=6.945]{64}
    \Vertex[L=$$,x=4.38,y=3.06]{65}
    \Vertex[L=$$,x=10.44,y=4.485]{66}
    \Vertex[L=$$,x=10.92,y=12.18]{67}
    \Vertex[L=$$,x=9.735,y=4.275]{68}
    \Vertex[L=$$,x=10.35,y=2.025]{69}
    \Vertex[L=$$,x=13.92,y=7.095]{70}
    \Vertex[L=$$,x=7.74,y=9.285]{71}
    \Vertex[L=$$,x=10.44,y=5.19]{72}
    \Vertex[L=$$,x=10.47,y=4.62]{73}
    \Vertex[L=$$,x=0.345,y=2.19]{74}
    \Vertex[L=$$,x=9.03,y=1.32]{75}
    \Vertex[L=$$,x=11.715,y=5.28]{76}
    \Vertex[L=$$,x=11.925,y=5.88]{77}
    \Vertex[L=$$,x=8.385,y=3.48]{78}
    \Vertex[L=$$,x=4.515,y=6.81]{79}
    \Vertex[L=$$,x=13.32,y=10.635]{80}
    \Vertex[L=$$,x=10.395,y=5.985]{81}
    \Vertex[L=$$,x=10.56,y=2.22]{82}
    \Vertex[L=$$,x=6.06,y=4.425]{83}
    \Vertex[L=$$,x=10.035,y=5.355]{84}
    \Vertex[L=$$,x=8.085,y=6.54]{85}
    \Vertex[L=$$,x=9.93,y=1.02]{86}
    \Vertex[L=$$,x=5.835,y=9.0]{87}
    \Vertex[L=$$,x=10.56,y=2.43]{88}
    \Vertex[L=$$,x=4.11,y=5.205]{89}
    \Vertex[L=$$,x=7.575,y=4.47]{90}
    \Vertex[L=$$,x=9.84,y=5.79]{91}
    \Vertex[L=$$,x=10.62,y=8.595]{92}
    \Vertex[L=$$,x=11.28,y=7.395]{93}
    \Vertex[L=$$,x=9.045,y=3.705]{94}
    \Vertex[L=$$,x=2.835,y=6.45]{95}
    \Vertex[L=$$,x=10.515,y=5.205]{96}
    \Vertex[L=$$,x=3.15,y=8.97]{97}
    \Vertex[L=$$,x=11.955,y=7.935]{98}
    \Vertex[L=$$,x=13.635,y=12.675]{99}
    \Vertex[L=$$,x=13.965,y=7.095]{100}
    \Vertex[L=$$,x=13.86,y=8.265]{101}
    \Vertex[L=$$,x=8.865,y=13.14]{102}
    \Vertex[L=$$,x=4.26,y=2.595]{103}
    \Vertex[L=$$,x=10.125,y=3.885]{104}
    \Vertex[L=$$,x=7.32,y=5.49]{105}
    \Vertex[L=$$,x=14.19,y=10.83]{106}
    \Vertex[L=$$,x=8.88,y=0.21]{107}
    \Vertex[L=$$,x=8.25,y=12.36]{108}
    \Vertex[L=$$,x=13.62,y=5.655]{109}
    \Vertex[L=$$,x=9.51,y=4.98]{110}
    \Vertex[L=$$,x=10.125,y=2.955]{111}
    \Vertex[L=$$,x=11.745,y=5.145]{112}
    \Vertex[L=$$,x=4.695,y=2.52]{113}
    \Vertex[L=$$,x=13.845,y=7.665]{114}
    \Vertex[L=$$,x=10.59,y=12.255]{115}
    \Vertex[L=$$,x=0.0,y=6.09]{116}
    \Vertex[L=$$,x=9.105,y=10.11]{117}
    \Vertex[L=$$,x=8.43,y=6.585]{118}
    \Vertex[L=$$,x=10.11,y=7.11]{119}
    \Vertex[L=$$,x=8.61,y=5.505]{120}
    \Vertex[L=$$,x=11.04,y=5.91]{121}
    \Vertex[L=$$,x=9.63,y=2.28]{122}
    \Vertex[L=$$,x=7.92,y=15.0]{123}
    \Vertex[L=$$,x=4.245,y=0.345]{124}
    \Vertex[L=$$,x=6.6,y=0.0]{125}
    \Vertex[L=$$,x=15.0,y=6.705]{126}
    \Vertex[L=$$,x=10.995,y=1.26]{127}
    \Vertex[L=$$,x=7.62,y=1.17]{128}
    \Vertex[L=$$,x=13.185,y=10.185]{129}
    \Vertex[L=$$,x=6.75,y=1.11]{130}
    \Vertex[L=$$,x=8.07,y=1.86]{131}
    \Vertex[L=$$,x=4.98,y=11.385]{132}
    \Vertex[L=$$,x=11.01,y=6.435]{133}
    \Vertex[L=$$,x=5.805,y=1.275]{134}
    \Vertex[L=$$,x=7.77,y=5.295]{135}
    \Vertex[L=$$,x=14.745,y=8.895]{136}
    \Vertex[L=$$,x=8.58,y=1.11]{137}
    \Vertex[L=$$,x=1.785,y=6.9]{138}
    \Vertex[L=$$,x=7.08,y=8.625]{139}
    \Vertex[L=$$,x=7.44,y=9.825]{140}
    \Vertex[L=$$,x=8.235,y=4.71]{141}
    \Vertex[L=$$,x=5.985,y=5.385]{142}
    \Vertex[L=$$,x=11.25,y=5.1]{143}
    \Vertex[L=$$,x=11.625,y=6.375]{144}
    \Vertex[L=$$,x=7.215,y=1.65]{145}
    \Vertex[L=$$,x=11.505,y=4.26]{146}
    \Vertex[L=$$,x=12.435,y=3.33]{147}
    \Vertex[L=$$,x=12.72,y=12.495]{148}
    \Vertex[L=$$,x=12.225,y=3.765]{149}
\AddVertexColor{gray!90, draw=black}{0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26,27,28,29,30,31,32,33,34,35,36,37,38,39,40,41,42,43,44,45,46,47,48,49,50,51,52,53,54,55,56,57,58,59,60,61,62,63,64,65,66,67,68,69,70,71,72,73,74,75,76,77,78,79,80,81,82,83,84,85,86,87,88,89,90,91,92,93,94,95,96,97,98,99,100,101,102,103,104,105,106,107,108,109,110,111,112,113,114,115,116,117,118,119,120,121,122,123,124,125,126,127,128,129,130,131,132,133,134,135,136,137,138,139,140,141,142,143,144,145,146,147,148,149}
\tikzstyle{EdgeStyle}=[line width=0.7pt, opacity = 0.3]
\tikzstyle{LabelStyle}=[fill=white]
    \Edge[label=](0)(2)
    \Edge[label=](0)(3)
    \Edge[label=](0)(7)
    \Edge[label=](0)(8)
    \Edge[label=](0)(9)
    \Edge[label=](0)(12)
    \Edge[label=](0)(13)
    \Edge[label=](0)(14)
    \Edge[label=](0)(17)
    \Edge[label=](0)(18)
    \Edge[label=](0)(23)
    \Edge[label=](0)(25)
    \Edge[label=](0)(31)
    \Edge[label=](0)(33)
    \Edge[label=](0)(36)
    \Edge[label=](0)(37)
    \Edge[label=](0)(64)
    \Edge[label=](0)(68)
    \Edge[label=](0)(75)
    \Edge[label=](0)(81)
    \Edge[label=](0)(82)
    \Edge[label=](0)(89)
    \Edge[label=](0)(95)
    \Edge[label=](0)(96)
    \Edge[label=](0)(98)
    \Edge[label=](0)(101)
    \Edge[label=](0)(108)
    \Edge[label=](1)(33)
    \Edge[label=](1)(2)
    \Edge[label=](1)(4)
    \Edge[label=](1)(5)
    \Edge[label=](1)(38)
    \Edge[label=](1)(15)
    \Edge[label=](1)(50)
    \Edge[label=](1)(52)
    \Edge[label=](1)(117)
    \Edge[label=](1)(118)
    \Edge[label=](1)(121)
    \Edge[label=](2)(3)
    \Edge[label=](2)(4)
    \Edge[label=](2)(5)
    \Edge[label=](2)(6)
    \Edge[label=](2)(135)
    \Edge[label=](2)(12)
    \Edge[label=](2)(16)
    \Edge[label=](2)(19)
    \Edge[label=](2)(21)
    \Edge[label=](2)(28)
    \Edge[label=](2)(34)
    \Edge[label=](2)(42)
    \Edge[label=](2)(48)
    \Edge[label=](2)(49)
    \Edge[label=](2)(51)
    \Edge[label=](2)(61)
    \Edge[label=](2)(72)
    \Edge[label=](2)(73)
    \Edge[label=](2)(91)
    \Edge[label=](2)(92)
    \Edge[label=](3)(36)
    \Edge[label=](3)(134)
    \Edge[label=](3)(7)
    \Edge[label=](3)(122)
    \Edge[label=](3)(11)
    \Edge[label=](3)(13)
    \Edge[label=](3)(66)
    \Edge[label=](3)(24)
    \Edge[label=](3)(68)
    \Edge[label=](3)(26)
    \Edge[label=](3)(29)
    \Edge[label=](3)(62)
    \Edge[label=](4)(118)
    \Edge[label=](4)(38)
    \Edge[label=](4)(138)
    \Edge[label=](4)(142)
    \Edge[label=](4)(79)
    \Edge[label=](4)(50)
    \Edge[label=](4)(19)
    \Edge[label=](4)(21)
    \Edge[label=](4)(22)
    \Edge[label=](4)(58)
    \Edge[label=](4)(59)
    \Edge[label=](4)(85)
    \Edge[label=](4)(53)
    \Edge[label=](5)(133)
    \Edge[label=](5)(6)
    \Edge[label=](5)(71)
    \Edge[label=](5)(139)
    \Edge[label=](5)(77)
    \Edge[label=](5)(87)
    \Edge[label=](5)(24)
    \Edge[label=](6)(70)
    \Edge[label=](6)(8)
    \Edge[label=](6)(9)
    \Edge[label=](6)(55)
    \Edge[label=](6)(141)
    \Edge[label=](6)(110)
    \Edge[label=](6)(15)
    \Edge[label=](6)(20)
    \Edge[label=](6)(23)
    \Edge[label=](6)(57)
    \Edge[label=](6)(47)
    \Edge[label=](7)(128)
    \Edge[label=](7)(130)
    \Edge[label=](7)(10)
    \Edge[label=](7)(145)
    \Edge[label=](7)(22)
    \Edge[label=](7)(25)
    \Edge[label=](7)(27)
    \Edge[label=](7)(37)
    \Edge[label=](7)(41)
    \Edge[label=](7)(42)
    \Edge[label=](7)(63)
    \Edge[label=](7)(65)
    \Edge[label=](7)(78)
    \Edge[label=](7)(90)
    \Edge[label=](7)(94)
    \Edge[label=](7)(103)
    \Edge[label=](7)(104)
    \Edge[label=](7)(111)
    \Edge[label=](7)(113)
    \Edge[label=](7)(124)
    \Edge[label=](8)(73)
    \Edge[label=](8)(10)
    \Edge[label=](8)(11)
    \Edge[label=](8)(76)
    \Edge[label=](8)(77)
    \Edge[label=](8)(146)
    \Edge[label=](8)(147)
    \Edge[label=](8)(63)
    \Edge[label=](9)(111)
    \Edge[label=](9)(147)
    \Edge[label=](9)(86)
    \Edge[label=](9)(127)
    \Edge[label=](10)(39)
    \Edge[label=](10)(109)
    \Edge[label=](10)(14)
    \Edge[label=](10)(112)
    \Edge[label=](10)(84)
    \Edge[label=](10)(27)
    \Edge[label=](11)(43)
    \Edge[label=](11)(60)
    \Edge[label=](12)(35)
    \Edge[label=](12)(133)
    \Edge[label=](12)(109)
    \Edge[label=](12)(45)
    \Edge[label=](12)(46)
    \Edge[label=](12)(47)
    \Edge[label=](12)(49)
    \Edge[label=](12)(114)
    \Edge[label=](12)(143)
    \Edge[label=](12)(28)
    \Edge[label=](12)(30)
    \Edge[label=](13)(34)
    \Edge[label=](13)(69)
    \Edge[label=](13)(72)
    \Edge[label=](13)(18)
    \Edge[label=](13)(20)
    \Edge[label=](14)(32)
    \Edge[label=](14)(35)
    \Edge[label=](14)(40)
    \Edge[label=](14)(64)
    \Edge[label=](14)(43)
    \Edge[label=](14)(44)
    \Edge[label=](14)(16)
    \Edge[label=](14)(140)
    \Edge[label=](14)(85)
    \Edge[label=](15)(66)
    \Edge[label=](15)(39)
    \Edge[label=](15)(51)
    \Edge[label=](15)(30)
    \Edge[label=](15)(31)
    \Edge[label=](16)(132)
    \Edge[label=](16)(102)
    \Edge[label=](16)(40)
    \Edge[label=](16)(44)
    \Edge[label=](16)(17)
    \Edge[label=](17)(48)
    \Edge[label=](17)(119)
    \Edge[label=](17)(140)
    \Edge[label=](17)(87)
    \Edge[label=](18)(70)
    \Edge[label=](18)(119)
    \Edge[label=](20)(104)
    \Edge[label=](20)(105)
    \Edge[label=](20)(75)
    \Edge[label=](20)(78)
    \Edge[label=](20)(143)
    \Edge[label=](20)(120)
    \Edge[label=](20)(29)
    \Edge[label=](21)(132)
    \Edge[label=](21)(139)
    \Edge[label=](21)(53)
    \Edge[label=](24)(115)
    \Edge[label=](25)(137)
    \Edge[label=](25)(26)
    \Edge[label=](26)(56)
    \Edge[label=](26)(55)
    \Edge[label=](26)(41)
    \Edge[label=](27)(69)
    \Edge[label=](27)(149)
    \Edge[label=](27)(54)
    \Edge[label=](27)(88)
    \Edge[label=](28)(32)
    \Edge[label=](30)(46)
    \Edge[label=](31)(90)
    \Edge[label=](32)(45)
    \Edge[label=](33)(76)
    \Edge[label=](35)(56)
    \Edge[label=](36)(65)
    \Edge[label=](36)(74)
    \Edge[label=](36)(113)
    \Edge[label=](37)(89)
    \Edge[label=](37)(135)
    \Edge[label=](37)(141)
    \Edge[label=](39)(144)
    \Edge[label=](39)(112)
    \Edge[label=](39)(52)
    \Edge[label=](39)(149)
    \Edge[label=](39)(54)
    \Edge[label=](39)(57)
    \Edge[label=](44)(108)
    \Edge[label=](45)(129)
    \Edge[label=](45)(67)
    \Edge[label=](48)(71)
    \Edge[label=](49)(88)
    \Edge[label=](50)(99)
    \Edge[label=](50)(148)
    \Edge[label=](50)(67)
    \Edge[label=](51)(80)
    \Edge[label=](51)(93)
    \Edge[label=](52)(96)
    \Edge[label=](52)(61)
    \Edge[label=](55)(131)
    \Edge[label=](55)(60)
    \Edge[label=](55)(59)
    \Edge[label=](55)(124)
    \Edge[label=](55)(62)
    \Edge[label=](56)(74)
    \Edge[label=](56)(58)
    \Edge[label=](56)(103)
    \Edge[label=](57)(131)
    \Edge[label=](59)(125)
    \Edge[label=](61)(110)
    \Edge[label=](61)(79)
    \Edge[label=](61)(81)
    \Edge[label=](61)(83)
    \Edge[label=](61)(84)
    \Edge[label=](63)(80)
    \Edge[label=](63)(136)
    \Edge[label=](63)(129)
    \Edge[label=](65)(83)
    \Edge[label=](67)(102)
    \Edge[label=](67)(144)
    \Edge[label=](67)(115)
    \Edge[label=](67)(92)
    \Edge[label=](69)(107)
    \Edge[label=](69)(122)
    \Edge[label=](70)(100)
    \Edge[label=](70)(101)
    \Edge[label=](70)(136)
    \Edge[label=](70)(126)
    \Edge[label=](73)(94)
    \Edge[label=](75)(128)
    \Edge[label=](75)(107)
    \Edge[label=](75)(82)
    \Edge[label=](75)(86)
    \Edge[label=](75)(125)
    \Edge[label=](77)(100)
    \Edge[label=](79)(97)
    \Edge[label=](79)(105)
    \Edge[label=](79)(95)
    \Edge[label=](80)(99)
    \Edge[label=](80)(98)
    \Edge[label=](81)(93)
    \Edge[label=](82)(127)
    \Edge[label=](84)(91)
    \Edge[label=](85)(120)
    \Edge[label=](87)(97)
    \Edge[label=](88)(137)
    \Edge[label=](89)(116)
    \Edge[label=](90)(142)
    \Edge[label=](95)(138)
    \Edge[label=](95)(116)
    \Edge[label=](99)(148)
    \Edge[label=](99)(106)
    \Edge[label=](101)(106)
    \Edge[label=](101)(114)
    \Edge[label=](102)(123)
    \Edge[label=](104)(146)
    \Edge[label=](108)(123)
    \Edge[label=](108)(117)
    \Edge[label=](109)(126)
    \Edge[label=](112)(121)
    \Edge[label=](124)(134)
    \Edge[label=](125)(130)
    \Edge[label=](128)(145)
\end{tikzpicture}
\label{dg}
\caption{Example Title}
\end{figure}


==> figures/visualizations/barabasi_2/diffusion_endpoint_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_2/diffusion_endpoint_3d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]
    \Vertex[L=$$,x=9.795,y=6.3]{0}
    \Vertex[L=$$,x=7.35,y=12.045]{1}
    \Vertex[L=$$,x=8.82,y=7.17]{2}
    \Vertex[L=$$,x=11.1,y=4.875]{3}
    \Vertex[L=$$,x=7.17,y=7.35]{4}
    \Vertex[L=$$,x=9.525,y=10.785]{5}
    \Vertex[L=$$,x=11.52,y=6.615]{6}
    \Vertex[L=$$,x=10.245,y=3.045]{7}
    \Vertex[L=$$,x=13.5,y=8.835]{8}
    \Vertex[L=$$,x=14.895,y=7.53]{9}
    \Vertex[L=$$,x=8.52,y=5.025]{10}
    \Vertex[L=$$,x=11.25,y=5.775]{11}
    \Vertex[L=$$,x=6.855,y=4.08]{12}
    \Vertex[L=$$,x=11.595,y=5.445]{13}
    \Vertex[L=$$,x=0.0,y=5.22]{14}
    \Vertex[L=$$,x=9.405,y=6.99]{15}
    \Vertex[L=$$,x=0.825,y=9.375]{16}
    \Vertex[L=$$,x=4.95,y=8.925]{17}
    \Vertex[L=$$,x=11.64,y=6.99]{18}
    \Vertex[L=$$,x=7.77,y=7.665]{19}
    \Vertex[L=$$,x=11.145,y=3.585]{20}
    \Vertex[L=$$,x=4.53,y=10.23]{21}
    \Vertex[L=$$,x=9.525,y=4.665]{22}
    \Vertex[L=$$,x=10.77,y=6.795]{23}
    \Vertex[L=$$,x=11.07,y=9.36]{24}
    \Vertex[L=$$,x=8.61,y=2.565]{25}
    \Vertex[L=$$,x=7.725,y=1.11]{26}
    \Vertex[L=$$,x=6.915,y=0.57]{27}
    \Vertex[L=$$,x=6.06,y=5.145]{28}
    \Vertex[L=$$,x=11.31,y=4.035]{29}
    \Vertex[L=$$,x=6.915,y=4.38]{30}
    \Vertex[L=$$,x=9.3,y=6.15]{31}
    \Vertex[L=$$,x=3.915,y=5.565]{32}
    \Vertex[L=$$,x=10.14,y=10.77]{33}
    \Vertex[L=$$,x=10.59,y=6.735]{34}
    \Vertex[L=$$,x=2.7,y=2.805]{35}
    \Vertex[L=$$,x=7.26,y=2.475]{36}
    \Vertex[L=$$,x=8.595,y=5.745]{37}
    \Vertex[L=$$,x=6.99,y=9.585]{38}
    \Vertex[L=$$,x=7.71,y=5.43]{39}
    \Vertex[L=$$,x=1.17,y=6.915]{40}
    \Vertex[L=$$,x=8.745,y=1.5]{41}
    \Vertex[L=$$,x=9.915,y=4.875]{42}
    \Vertex[L=$$,x=7.08,y=4.92]{43}
    \Vertex[L=$$,x=2.1,y=8.805]{44}
    \Vertex[L=$$,x=8.775,y=7.245]{45}
    \Vertex[L=$$,x=5.685,y=3.42]{46}
    \Vertex[L=$$,x=9.21,y=4.92]{47}
    \Vertex[L=$$,x=7.14,y=9.69]{48}
    \Vertex[L=$$,x=7.275,y=3.63]{49}
    \Vertex[L=$$,x=9.915,y=12.9]{50}
    \Vertex[L=$$,x=10.32,y=10.695]{51}
    \Vertex[L=$$,x=7.2,y=8.73]{52}
    \Vertex[L=$$,x=5.055,y=9.135]{53}
    \Vertex[L=$$,x=7.14,y=3.27]{54}
    \Vertex[L=$$,x=11.445,y=2.64]{55}
    \Vertex[L=$$,x=1.92,y=0.0]{56}
    \Vertex[L=$$,x=10.2,y=5.145]{57}
    \Vertex[L=$$,x=4.965,y=3.99]{58}
    \Vertex[L=$$,x=10.665,y=4.665]{59}
    \Vertex[L=$$,x=11.43,y=3.975]{60}
    \Vertex[L=$$,x=5.475,y=8.745]{61}
    \Vertex[L=$$,x=11.61,y=3.555]{62}
    \Vertex[L=$$,x=12.975,y=8.205]{63}
    \Vertex[L=$$,x=5.79,y=5.715]{64}
    \Vertex[L=$$,x=7.005,y=3.12]{65}
    \Vertex[L=$$,x=10.965,y=5.88]{66}
    \Vertex[L=$$,x=7.365,y=14.1]{67}
    \Vertex[L=$$,x=10.695,y=5.595]{68}
    \Vertex[L=$$,x=11.145,y=1.995]{69}
    \Vertex[L=$$,x=14.775,y=8.325]{70}
    \Vertex[L=$$,x=8.4,y=11.115]{71}
    \Vertex[L=$$,x=10.59,y=6.345]{72}
    \Vertex[L=$$,x=11.94,y=7.485]{73}
    \Vertex[L=$$,x=3.93,y=0.915]{74}
    \Vertex[L=$$,x=14.37,y=3.78]{75}
    \Vertex[L=$$,x=12.375,y=10.44]{76}
    \Vertex[L=$$,x=12.99,y=10.515]{77}
    \Vertex[L=$$,x=10.44,y=2.58]{78}
    \Vertex[L=$$,x=2.58,y=9.18]{79}
    \Vertex[L=$$,x=12.975,y=13.32]{80}
    \Vertex[L=$$,x=8.295,y=10.29]{81}
    \Vertex[L=$$,x=13.485,y=6.195]{82}
    \Vertex[L=$$,x=5.91,y=5.79]{83}
    \Vertex[L=$$,x=5.43,y=7.035]{84}
    \Vertex[L=$$,x=5.94,y=5.16]{85}
    \Vertex[L=$$,x=15.0,y=6.405]{86}
    \Vertex[L=$$,x=6.09,y=10.23]{87}
    \Vertex[L=$$,x=5.43,y=0.375]{88}
    \Vertex[L=$$,x=6.39,y=6.72]{89}
    \Vertex[L=$$,x=8.865,y=4.695]{90}
    \Vertex[L=$$,x=6.81,y=7.605]{91}
    \Vertex[L=$$,x=8.43,y=10.71]{92}
    \Vertex[L=$$,x=9.06,y=13.29]{93}
    \Vertex[L=$$,x=11.16,y=4.845]{94}
    \Vertex[L=$$,x=2.4,y=8.67]{95}
    \Vertex[L=$$,x=8.475,y=7.83]{96}
    \Vertex[L=$$,x=3.825,y=9.855]{97}
    \Vertex[L=$$,x=11.265,y=9.345]{98}
    \Vertex[L=$$,x=12.735,y=15.0]{99}
    \Vertex[L=$$,x=14.4,y=9.345]{100}
    \Vertex[L=$$,x=12.99,y=8.16]{101}
    \Vertex[L=$$,x=4.83,y=12.645]{102}
    \Vertex[L=$$,x=6.765,y=1.545]{103}
    \Vertex[L=$$,x=12.21,y=4.2]{104}
    \Vertex[L=$$,x=8.685,y=5.655]{105}
    \Vertex[L=$$,x=13.2,y=10.98]{106}
    \Vertex[L=$$,x=13.245,y=2.91]{107}
    \Vertex[L=$$,x=4.02,y=11.475]{108}
    \Vertex[L=$$,x=9.135,y=4.065]{109}
    \Vertex[L=$$,x=8.805,y=7.275]{110}
    \Vertex[L=$$,x=12.57,y=4.905]{111}
    \Vertex[L=$$,x=7.14,y=6.45]{112}
    \Vertex[L=$$,x=8.265,y=1.785]{113}
    \Vertex[L=$$,x=10.395,y=5.475]{114}
    \Vertex[L=$$,x=9.27,y=13.155]{115}
    \Vertex[L=$$,x=1.68,y=8.19]{116}
    \Vertex[L=$$,x=5.295,y=12.24]{117}
    \Vertex[L=$$,x=6.855,y=10.14]{118}
    \Vertex[L=$$,x=8.115,y=7.335]{119}
    \Vertex[L=$$,x=9.27,y=3.96]{120}
    \Vertex[L=$$,x=7.32,y=9.135]{121}
    \Vertex[L=$$,x=11.73,y=3.075]{122}
    \Vertex[L=$$,x=3.87,y=12.645]{123}
    \Vertex[L=$$,x=11.655,y=2.85]{124}
    \Vertex[L=$$,x=13.44,y=3.585]{125}
    \Vertex[L=$$,x=12.795,y=5.595]{126}
    \Vertex[L=$$,x=14.79,y=7.665]{127}
    \Vertex[L=$$,x=12.165,y=2.55]{128}
    \Vertex[L=$$,x=11.265,y=7.965]{129}
    \Vertex[L=$$,x=11.565,y=2.7]{130}
    \Vertex[L=$$,x=10.95,y=3.36]{131}
    \Vertex[L=$$,x=2.13,y=10.065]{132}
    \Vertex[L=$$,x=8.985,y=6.615]{133}
    \Vertex[L=$$,x=11.94,y=4.14]{134}
    \Vertex[L=$$,x=8.55,y=6.675]{135}
    \Vertex[L=$$,x=14.175,y=8.475]{136}
    \Vertex[L=$$,x=6.225,y=0.9]{137}
    \Vertex[L=$$,x=4.26,y=8.1]{138}
    \Vertex[L=$$,x=7.08,y=10.65]{139}
    \Vertex[L=$$,x=2.79,y=6.645]{140}
    \Vertex[L=$$,x=9.45,y=6.195]{141}
    \Vertex[L=$$,x=7.365,y=6.105]{142}
    \Vertex[L=$$,x=9.24,y=3.345]{143}
    \Vertex[L=$$,x=8.49,y=8.37]{144}
    \Vertex[L=$$,x=10.92,y=2.535]{145}
    \Vertex[L=$$,x=13.605,y=7.17]{146}
    \Vertex[L=$$,x=14.805,y=8.805]{147}
    \Vertex[L=$$,x=11.88,y=13.605]{148}
    \Vertex[L=$$,x=7.035,y=3.165]{149}
\AddVertexColor{gray!90, draw=black}{0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26,27,28,29,30,31,32,33,34,35,36,37,38,39,40,41,42,43,44,45,46,47,48,49,50,51,52,53,54,55,56,57,58,59,60,61,62,63,64,65,66,67,68,69,70,71,72,73,74,75,76,77,78,79,80,81,82,83,84,85,86,87,88,89,90,91,92,93,94,95,96,97,98,99,100,101,102,103,104,105,106,107,108,109,110,111,112,113,114,115,116,117,118,119,120,121,122,123,124,125,126,127,128,129,130,131,132,133,134,135,136,137,138,139,140,141,142,143,144,145,146,147,148,149}
\tikzstyle{EdgeStyle}=[line width=0.7pt, opacity = 0.3]
\tikzstyle{LabelStyle}=[fill=white]
    \Edge[label=](0)(2)
    \Edge[label=](0)(3)
    \Edge[label=](0)(7)
    \Edge[label=](0)(8)
    \Edge[label=](0)(9)
    \Edge[label=](0)(12)
    \Edge[label=](0)(13)
    \Edge[label=](0)(14)
    \Edge[label=](0)(17)
    \Edge[label=](0)(18)
    \Edge[label=](0)(23)
    \Edge[label=](0)(25)
    \Edge[label=](0)(31)
    \Edge[label=](0)(33)
    \Edge[label=](0)(36)
    \Edge[label=](0)(37)
    \Edge[label=](0)(64)
    \Edge[label=](0)(68)
    \Edge[label=](0)(75)
    \Edge[label=](0)(81)
    \Edge[label=](0)(82)
    \Edge[label=](0)(89)
    \Edge[label=](0)(95)
    \Edge[label=](0)(96)
    \Edge[label=](0)(98)
    \Edge[label=](0)(101)
    \Edge[label=](0)(108)
    \Edge[label=](1)(33)
    \Edge[label=](1)(2)
    \Edge[label=](1)(4)
    \Edge[label=](1)(5)
    \Edge[label=](1)(38)
    \Edge[label=](1)(15)
    \Edge[label=](1)(50)
    \Edge[label=](1)(52)
    \Edge[label=](1)(117)
    \Edge[label=](1)(118)
    \Edge[label=](1)(121)
    \Edge[label=](2)(3)
    \Edge[label=](2)(4)
    \Edge[label=](2)(5)
    \Edge[label=](2)(6)
    \Edge[label=](2)(135)
    \Edge[label=](2)(12)
    \Edge[label=](2)(16)
    \Edge[label=](2)(19)
    \Edge[label=](2)(21)
    \Edge[label=](2)(28)
    \Edge[label=](2)(34)
    \Edge[label=](2)(42)
    \Edge[label=](2)(48)
    \Edge[label=](2)(49)
    \Edge[label=](2)(51)
    \Edge[label=](2)(61)
    \Edge[label=](2)(72)
    \Edge[label=](2)(73)
    \Edge[label=](2)(91)
    \Edge[label=](2)(92)
    \Edge[label=](3)(36)
    \Edge[label=](3)(134)
    \Edge[label=](3)(7)
    \Edge[label=](3)(122)
    \Edge[label=](3)(11)
    \Edge[label=](3)(13)
    \Edge[label=](3)(66)
    \Edge[label=](3)(24)
    \Edge[label=](3)(68)
    \Edge[label=](3)(26)
    \Edge[label=](3)(29)
    \Edge[label=](3)(62)
    \Edge[label=](4)(118)
    \Edge[label=](4)(38)
    \Edge[label=](4)(138)
    \Edge[label=](4)(142)
    \Edge[label=](4)(79)
    \Edge[label=](4)(50)
    \Edge[label=](4)(19)
    \Edge[label=](4)(21)
    \Edge[label=](4)(22)
    \Edge[label=](4)(58)
    \Edge[label=](4)(59)
    \Edge[label=](4)(85)
    \Edge[label=](4)(53)
    \Edge[label=](5)(133)
    \Edge[label=](5)(6)
    \Edge[label=](5)(71)
    \Edge[label=](5)(139)
    \Edge[label=](5)(77)
    \Edge[label=](5)(87)
    \Edge[label=](5)(24)
    \Edge[label=](6)(70)
    \Edge[label=](6)(8)
    \Edge[label=](6)(9)
    \Edge[label=](6)(55)
    \Edge[label=](6)(141)
    \Edge[label=](6)(110)
    \Edge[label=](6)(15)
    \Edge[label=](6)(20)
    \Edge[label=](6)(23)
    \Edge[label=](6)(57)
    \Edge[label=](6)(47)
    \Edge[label=](7)(128)
    \Edge[label=](7)(130)
    \Edge[label=](7)(10)
    \Edge[label=](7)(145)
    \Edge[label=](7)(22)
    \Edge[label=](7)(25)
    \Edge[label=](7)(27)
    \Edge[label=](7)(37)
    \Edge[label=](7)(41)
    \Edge[label=](7)(42)
    \Edge[label=](7)(63)
    \Edge[label=](7)(65)
    \Edge[label=](7)(78)
    \Edge[label=](7)(90)
    \Edge[label=](7)(94)
    \Edge[label=](7)(103)
    \Edge[label=](7)(104)
    \Edge[label=](7)(111)
    \Edge[label=](7)(113)
    \Edge[label=](7)(124)
    \Edge[label=](8)(73)
    \Edge[label=](8)(10)
    \Edge[label=](8)(11)
    \Edge[label=](8)(76)
    \Edge[label=](8)(77)
    \Edge[label=](8)(146)
    \Edge[label=](8)(147)
    \Edge[label=](8)(63)
    \Edge[label=](9)(111)
    \Edge[label=](9)(147)
    \Edge[label=](9)(86)
    \Edge[label=](9)(127)
    \Edge[label=](10)(39)
    \Edge[label=](10)(109)
    \Edge[label=](10)(14)
    \Edge[label=](10)(112)
    \Edge[label=](10)(84)
    \Edge[label=](10)(27)
    \Edge[label=](11)(43)
    \Edge[label=](11)(60)
    \Edge[label=](12)(35)
    \Edge[label=](12)(133)
    \Edge[label=](12)(109)
    \Edge[label=](12)(45)
    \Edge[label=](12)(46)
    \Edge[label=](12)(47)
    \Edge[label=](12)(49)
    \Edge[label=](12)(114)
    \Edge[label=](12)(143)
    \Edge[label=](12)(28)
    \Edge[label=](12)(30)
    \Edge[label=](13)(34)
    \Edge[label=](13)(69)
    \Edge[label=](13)(72)
    \Edge[label=](13)(18)
    \Edge[label=](13)(20)
    \Edge[label=](14)(32)
    \Edge[label=](14)(35)
    \Edge[label=](14)(40)
    \Edge[label=](14)(64)
    \Edge[label=](14)(43)
    \Edge[label=](14)(44)
    \Edge[label=](14)(16)
    \Edge[label=](14)(140)
    \Edge[label=](14)(85)
    \Edge[label=](15)(66)
    \Edge[label=](15)(39)
    \Edge[label=](15)(51)
    \Edge[label=](15)(30)
    \Edge[label=](15)(31)
    \Edge[label=](16)(132)
    \Edge[label=](16)(102)
    \Edge[label=](16)(40)
    \Edge[label=](16)(44)
    \Edge[label=](16)(17)
    \Edge[label=](17)(48)
    \Edge[label=](17)(119)
    \Edge[label=](17)(140)
    \Edge[label=](17)(87)
    \Edge[label=](18)(70)
    \Edge[label=](18)(119)
    \Edge[label=](20)(104)
    \Edge[label=](20)(105)
    \Edge[label=](20)(75)
    \Edge[label=](20)(78)
    \Edge[label=](20)(143)
    \Edge[label=](20)(120)
    \Edge[label=](20)(29)
    \Edge[label=](21)(132)
    \Edge[label=](21)(139)
    \Edge[label=](21)(53)
    \Edge[label=](24)(115)
    \Edge[label=](25)(137)
    \Edge[label=](25)(26)
    \Edge[label=](26)(56)
    \Edge[label=](26)(55)
    \Edge[label=](26)(41)
    \Edge[label=](27)(69)
    \Edge[label=](27)(149)
    \Edge[label=](27)(54)
    \Edge[label=](27)(88)
    \Edge[label=](28)(32)
    \Edge[label=](30)(46)
    \Edge[label=](31)(90)
    \Edge[label=](32)(45)
    \Edge[label=](33)(76)
    \Edge[label=](35)(56)
    \Edge[label=](36)(65)
    \Edge[label=](36)(74)
    \Edge[label=](36)(113)
    \Edge[label=](37)(89)
    \Edge[label=](37)(135)
    \Edge[label=](37)(141)
    \Edge[label=](39)(144)
    \Edge[label=](39)(112)
    \Edge[label=](39)(52)
    \Edge[label=](39)(149)
    \Edge[label=](39)(54)
    \Edge[label=](39)(57)
    \Edge[label=](44)(108)
    \Edge[label=](45)(129)
    \Edge[label=](45)(67)
    \Edge[label=](48)(71)
    \Edge[label=](49)(88)
    \Edge[label=](50)(99)
    \Edge[label=](50)(148)
    \Edge[label=](50)(67)
    \Edge[label=](51)(80)
    \Edge[label=](51)(93)
    \Edge[label=](52)(96)
    \Edge[label=](52)(61)
    \Edge[label=](55)(131)
    \Edge[label=](55)(60)
    \Edge[label=](55)(59)
    \Edge[label=](55)(124)
    \Edge[label=](55)(62)
    \Edge[label=](56)(74)
    \Edge[label=](56)(58)
    \Edge[label=](56)(103)
    \Edge[label=](57)(131)
    \Edge[label=](59)(125)
    \Edge[label=](61)(110)
    \Edge[label=](61)(79)
    \Edge[label=](61)(81)
    \Edge[label=](61)(83)
    \Edge[label=](61)(84)
    \Edge[label=](63)(80)
    \Edge[label=](63)(136)
    \Edge[label=](63)(129)
    \Edge[label=](65)(83)
    \Edge[label=](67)(102)
    \Edge[label=](67)(144)
    \Edge[label=](67)(115)
    \Edge[label=](67)(92)
    \Edge[label=](69)(107)
    \Edge[label=](69)(122)
    \Edge[label=](70)(100)
    \Edge[label=](70)(101)
    \Edge[label=](70)(136)
    \Edge[label=](70)(126)
    \Edge[label=](73)(94)
    \Edge[label=](75)(128)
    \Edge[label=](75)(107)
    \Edge[label=](75)(82)
    \Edge[label=](75)(86)
    \Edge[label=](75)(125)
    \Edge[label=](77)(100)
    \Edge[label=](79)(97)
    \Edge[label=](79)(105)
    \Edge[label=](79)(95)
    \Edge[label=](80)(99)
    \Edge[label=](80)(98)
    \Edge[label=](81)(93)
    \Edge[label=](82)(127)
    \Edge[label=](84)(91)
    \Edge[label=](85)(120)
    \Edge[label=](87)(97)
    \Edge[label=](88)(137)
    \Edge[label=](89)(116)
    \Edge[label=](90)(142)
    \Edge[label=](95)(138)
    \Edge[label=](95)(116)
    \Edge[label=](99)(148)
    \Edge[label=](99)(106)
    \Edge[label=](101)(106)
    \Edge[label=](101)(114)
    \Edge[label=](102)(123)
    \Edge[label=](104)(146)
    \Edge[label=](108)(123)
    \Edge[label=](108)(117)
    \Edge[label=](109)(126)
    \Edge[label=](112)(121)
    \Edge[label=](124)(134)
    \Edge[label=](125)(130)
    \Edge[label=](128)(145)
\end{tikzpicture}
\label{dg}
\caption{Example Title}
\end{figure}


==> figures/visualizations/barabasi_2/node2vec_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/barabasi_2/node2vec_3d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]
    \Vertex[L=$$,x=9.195,y=4.725]{0}
    \Vertex[L=$$,x=8.22,y=6.39]{1}
    \Vertex[L=$$,x=8.49,y=5.745]{2}
    \Vertex[L=$$,x=7.92,y=3.555]{3}
    \Vertex[L=$$,x=4.41,y=5.28]{4}
    \Vertex[L=$$,x=7.905,y=6.675]{5}
    \Vertex[L=$$,x=10.035,y=4.605]{6}
    \Vertex[L=$$,x=7.845,y=2.925]{7}
    \Vertex[L=$$,x=11.085,y=4.845]{8}
    \Vertex[L=$$,x=11.025,y=2.805]{9}
    \Vertex[L=$$,x=10.635,y=4.89]{10}
    \Vertex[L=$$,x=8.655,y=4.05]{11}
    \Vertex[L=$$,x=11.265,y=6.51]{12}
    \Vertex[L=$$,x=9.645,y=4.245]{13}
    \Vertex[L=$$,x=7.59,y=6.75]{14}
    \Vertex[L=$$,x=10.41,y=5.55]{15}
    \Vertex[L=$$,x=5.16,y=9.42]{16}
    \Vertex[L=$$,x=5.19,y=8.085]{17}
    \Vertex[L=$$,x=10.515,y=5.565]{18}
    \Vertex[L=$$,x=6.48,y=5.505]{19}
    \Vertex[L=$$,x=8.475,y=3.735]{20}
    \Vertex[L=$$,x=3.435,y=7.2]{21}
    \Vertex[L=$$,x=6.315,y=3.9]{22}
    \Vertex[L=$$,x=9.57,y=4.695]{23}
    \Vertex[L=$$,x=8.835,y=5.985]{24}
    \Vertex[L=$$,x=8.985,y=2.97]{25}
    \Vertex[L=$$,x=5.535,y=2.025]{26}
    \Vertex[L=$$,x=12.195,y=3.63]{27}
    \Vertex[L=$$,x=10.155,y=7.035]{28}
    \Vertex[L=$$,x=8.115,y=3.465]{29}
    \Vertex[L=$$,x=12.21,y=6.885]{30}
    \Vertex[L=$$,x=8.715,y=4.635]{31}
    \Vertex[L=$$,x=9.825,y=8.715]{32}
    \Vertex[L=$$,x=9.54,y=5.325]{33}
    \Vertex[L=$$,x=9.135,y=4.935]{34}
    \Vertex[L=$$,x=8.22,y=4.815]{35}
    \Vertex[L=$$,x=4.83,y=2.76]{36}
    \Vertex[L=$$,x=7.395,y=4.17]{37}
    \Vertex[L=$$,x=6.585,y=5.88]{38}
    \Vertex[L=$$,x=11.865,y=5.355]{39}
    \Vertex[L=$$,x=5.76,y=8.955]{40}
    \Vertex[L=$$,x=6.03,y=2.04]{41}
    \Vertex[L=$$,x=8.565,y=4.23]{42}
    \Vertex[L=$$,x=8.175,y=5.205]{43}
    \Vertex[L=$$,x=5.4,y=9.765]{44}
    \Vertex[L=$$,x=11.265,y=9.675]{45}
    \Vertex[L=$$,x=12.705,y=7.365]{46}
    \Vertex[L=$$,x=10.905,y=5.37]{47}
    \Vertex[L=$$,x=5.805,y=7.905]{48}
    \Vertex[L=$$,x=11.13,y=5.145]{49}
    \Vertex[L=$$,x=9.345,y=8.085]{50}
    \Vertex[L=$$,x=10.44,y=6.6]{51}
    \Vertex[L=$$,x=9.0,y=5.445]{52}
    \Vertex[L=$$,x=2.52,y=6.435]{53}
    \Vertex[L=$$,x=12.915,y=4.455]{54}
    \Vertex[L=$$,x=6.63,y=2.13]{55}
    \Vertex[L=$$,x=1.32,y=2.355]{56}
    \Vertex[L=$$,x=10.875,y=4.065]{57}
    \Vertex[L=$$,x=2.265,y=3.81]{58}
    \Vertex[L=$$,x=5.985,y=2.895]{59}
    \Vertex[L=$$,x=7.455,y=3.015]{60}
    \Vertex[L=$$,x=6.705,y=5.04]{61}
    \Vertex[L=$$,x=6.81,y=2.475]{62}
    \Vertex[L=$$,x=12.09,y=5.805]{63}
    \Vertex[L=$$,x=8.58,y=5.685]{64}
    \Vertex[L=$$,x=4.86,y=2.715]{65}
    \Vertex[L=$$,x=9.48,y=4.455]{66}
    \Vertex[L=$$,x=9.255,y=12.12]{67}
    \Vertex[L=$$,x=8.535,y=4.14]{68}
    \Vertex[L=$$,x=11.4,y=2.775]{69}
    \Vertex[L=$$,x=13.68,y=6.69]{70}
    \Vertex[L=$$,x=5.685,y=8.01]{71}
    \Vertex[L=$$,x=9.21,y=4.92]{72}
    \Vertex[L=$$,x=9.57,y=4.575]{73}
    \Vertex[L=$$,x=0.0,y=1.71]{74}
    \Vertex[L=$$,x=8.91,y=1.635]{75}
    \Vertex[L=$$,x=10.725,y=5.115]{76}
    \Vertex[L=$$,x=10.86,y=5.955]{77}
    \Vertex[L=$$,x=8.205,y=3.27]{78}
    \Vertex[L=$$,x=1.92,y=5.295]{79}
    \Vertex[L=$$,x=12.36,y=8.79]{80}
    \Vertex[L=$$,x=8.685,y=5.28]{81}
    \Vertex[L=$$,x=10.47,y=2.445]{82}
    \Vertex[L=$$,x=4.815,y=3.645]{83}
    \Vertex[L=$$,x=8.475,y=5.19]{84}
    \Vertex[L=$$,x=6.015,y=5.385]{85}
    \Vertex[L=$$,x=10.23,y=1.605]{86}
    \Vertex[L=$$,x=3.165,y=7.86]{87}
    \Vertex[L=$$,x=12.51,y=3.825]{88}
    \Vertex[L=$$,x=5.625,y=4.35]{89}
    \Vertex[L=$$,x=6.3,y=3.645]{90}
    \Vertex[L=$$,x=8.46,y=5.52]{91}
    \Vertex[L=$$,x=9.12,y=7.86]{92}
    \Vertex[L=$$,x=9.825,y=6.24]{93}
    \Vertex[L=$$,x=8.79,y=3.6]{94}
    \Vertex[L=$$,x=1.695,y=5.01]{95}
    \Vertex[L=$$,x=9.03,y=5.22]{96}
    \Vertex[L=$$,x=0.33,y=7.14]{97}
    \Vertex[L=$$,x=10.83,y=6.12]{98}
    \Vertex[L=$$,x=12.06,y=12.645]{99}
    \Vertex[L=$$,x=12.99,y=6.69]{100}
    \Vertex[L=$$,x=13.02,y=7.485]{101}
    \Vertex[L=$$,x=5.91,y=13.29]{102}
    \Vertex[L=$$,x=4.5,y=2.355]{103}
    \Vertex[L=$$,x=9.135,y=3.225]{104}
    \Vertex[L=$$,x=5.46,y=4.275]{105}
    \Vertex[L=$$,x=13.89,y=11.775]{106}
    \Vertex[L=$$,x=10.44,y=1.635]{107}
    \Vertex[L=$$,x=6.78,y=9.3]{108}
    \Vertex[L=$$,x=13.08,y=6.285]{109}
    \Vertex[L=$$,x=8.385,y=4.725]{110}
    \Vertex[L=$$,x=9.42,y=2.565]{111}
    \Vertex[L=$$,x=11.13,y=5.55]{112}
    \Vertex[L=$$,x=5.4,y=2.235]{113}
    \Vertex[L=$$,x=12.87,y=7.62]{114}
    \Vertex[L=$$,x=8.565,y=10.59]{115}
    \Vertex[L=$$,x=1.38,y=4.56]{116}
    \Vertex[L=$$,x=6.99,y=8.325]{117}
    \Vertex[L=$$,x=6.555,y=5.865]{118}
    \Vertex[L=$$,x=8.61,y=6.33]{119}
    \Vertex[L=$$,x=7.11,y=4.44]{120}
    \Vertex[L=$$,x=10.05,y=6.03]{121}
    \Vertex[L=$$,x=10.02,y=2.85]{122}
    \Vertex[L=$$,x=4.47,y=15.0]{123}
    \Vertex[L=$$,x=6.0,y=1.545]{124}
    \Vertex[L=$$,x=5.37,y=0.0]{125}
    \Vertex[L=$$,x=15.0,y=7.275]{126}
    \Vertex[L=$$,x=11.265,y=2.085]{127}
    \Vertex[L=$$,x=7.305,y=1.035]{128}
    \Vertex[L=$$,x=12.6,y=9.225]{129}
    \Vertex[L=$$,x=5.805,y=0.915]{130}
    \Vertex[L=$$,x=9.3,y=3.06]{131}
    \Vertex[L=$$,x=2.775,y=9.48]{132}
    \Vertex[L=$$,x=9.39,y=6.645]{133}
    \Vertex[L=$$,x=6.135,y=2.025]{134}
    \Vertex[L=$$,x=7.845,y=4.98]{135}
    \Vertex[L=$$,x=14.61,y=7.59]{136}
    \Vertex[L=$$,x=11.13,y=2.925]{137}
    \Vertex[L=$$,x=0.96,y=5.43]{138}
    \Vertex[L=$$,x=5.1,y=7.335]{139}
    \Vertex[L=$$,x=5.535,y=8.025]{140}
    \Vertex[L=$$,x=8.64,y=4.35]{141}
    \Vertex[L=$$,x=4.44,y=4.38]{142}
    \Vertex[L=$$,x=10.17,y=4.92]{143}
    \Vertex[L=$$,x=11.16,y=7.485]{144}
    \Vertex[L=$$,x=6.915,y=1.185]{145}
    \Vertex[L=$$,x=10.47,y=3.795]{146}
    \Vertex[L=$$,x=11.88,y=3.66]{147}
    \Vertex[L=$$,x=10.845,y=13.455]{148}
    \Vertex[L=$$,x=12.945,y=4.44]{149}
\AddVertexColor{gray!90, draw=black}{0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26,27,28,29,30,31,32,33,34,35,36,37,38,39,40,41,42,43,44,45,46,47,48,49,50,51,52,53,54,55,56,57,58,59,60,61,62,63,64,65,66,67,68,69,70,71,72,73,74,75,76,77,78,79,80,81,82,83,84,85,86,87,88,89,90,91,92,93,94,95,96,97,98,99,100,101,102,103,104,105,106,107,108,109,110,111,112,113,114,115,116,117,118,119,120,121,122,123,124,125,126,127,128,129,130,131,132,133,134,135,136,137,138,139,140,141,142,143,144,145,146,147,148,149}
\tikzstyle{EdgeStyle}=[line width=0.7pt, opacity = 0.3]
\tikzstyle{LabelStyle}=[fill=white]
    \Edge[label=](0)(2)
    \Edge[label=](0)(3)
    \Edge[label=](0)(7)
    \Edge[label=](0)(8)
    \Edge[label=](0)(9)
    \Edge[label=](0)(12)
    \Edge[label=](0)(13)
    \Edge[label=](0)(14)
    \Edge[label=](0)(17)
    \Edge[label=](0)(18)
    \Edge[label=](0)(23)
    \Edge[label=](0)(25)
    \Edge[label=](0)(31)
    \Edge[label=](0)(33)
    \Edge[label=](0)(36)
    \Edge[label=](0)(37)
    \Edge[label=](0)(64)
    \Edge[label=](0)(68)
    \Edge[label=](0)(75)
    \Edge[label=](0)(81)
    \Edge[label=](0)(82)
    \Edge[label=](0)(89)
    \Edge[label=](0)(95)
    \Edge[label=](0)(96)
    \Edge[label=](0)(98)
    \Edge[label=](0)(101)
    \Edge[label=](0)(108)
    \Edge[label=](1)(33)
    \Edge[label=](1)(2)
    \Edge[label=](1)(4)
    \Edge[label=](1)(5)
    \Edge[label=](1)(38)
    \Edge[label=](1)(15)
    \Edge[label=](1)(50)
    \Edge[label=](1)(52)
    \Edge[label=](1)(117)
    \Edge[label=](1)(118)
    \Edge[label=](1)(121)
    \Edge[label=](2)(3)
    \Edge[label=](2)(4)
    \Edge[label=](2)(5)
    \Edge[label=](2)(6)
    \Edge[label=](2)(135)
    \Edge[label=](2)(12)
    \Edge[label=](2)(16)
    \Edge[label=](2)(19)
    \Edge[label=](2)(21)
    \Edge[label=](2)(28)
    \Edge[label=](2)(34)
    \Edge[label=](2)(42)
    \Edge[label=](2)(48)
    \Edge[label=](2)(49)
    \Edge[label=](2)(51)
    \Edge[label=](2)(61)
    \Edge[label=](2)(72)
    \Edge[label=](2)(73)
    \Edge[label=](2)(91)
    \Edge[label=](2)(92)
    \Edge[label=](3)(36)
    \Edge[label=](3)(134)
    \Edge[label=](3)(7)
    \Edge[label=](3)(122)
    \Edge[label=](3)(11)
    \Edge[label=](3)(13)
    \Edge[label=](3)(66)
    \Edge[label=](3)(24)
    \Edge[label=](3)(68)
    \Edge[label=](3)(26)
    \Edge[label=](3)(29)
    \Edge[label=](3)(62)
    \Edge[label=](4)(118)
    \Edge[label=](4)(38)
    \Edge[label=](4)(138)
    \Edge[label=](4)(142)
    \Edge[label=](4)(79)
    \Edge[label=](4)(50)
    \Edge[label=](4)(19)
    \Edge[label=](4)(21)
    \Edge[label=](4)(22)
    \Edge[label=](4)(58)
    \Edge[label=](4)(59)
    \Edge[label=](4)(85)
    \Edge[label=](4)(53)
    \Edge[label=](5)(133)
    \Edge[label=](5)(6)
    \Edge[label=](5)(71)
    \Edge[label=](5)(139)
    \Edge[label=](5)(77)
    \Edge[label=](5)(87)
    \Edge[label=](5)(24)
    \Edge[label=](6)(70)
    \Edge[label=](6)(8)
    \Edge[label=](6)(9)
    \Edge[label=](6)(55)
    \Edge[label=](6)(141)
    \Edge[label=](6)(110)
    \Edge[label=](6)(15)
    \Edge[label=](6)(20)
    \Edge[label=](6)(23)
    \Edge[label=](6)(57)
    \Edge[label=](6)(47)
    \Edge[label=](7)(128)
    \Edge[label=](7)(130)
    \Edge[label=](7)(10)
    \Edge[label=](7)(145)
    \Edge[label=](7)(22)
    \Edge[label=](7)(25)
    \Edge[label=](7)(27)
    \Edge[label=](7)(37)
    \Edge[label=](7)(41)
    \Edge[label=](7)(42)
    \Edge[label=](7)(63)
    \Edge[label=](7)(65)
    \Edge[label=](7)(78)
    \Edge[label=](7)(90)
    \Edge[label=](7)(94)
    \Edge[label=](7)(103)
    \Edge[label=](7)(104)
    \Edge[label=](7)(111)
    \Edge[label=](7)(113)
    \Edge[label=](7)(124)
    \Edge[label=](8)(73)
    \Edge[label=](8)(10)
    \Edge[label=](8)(11)
    \Edge[label=](8)(76)
    \Edge[label=](8)(77)
    \Edge[label=](8)(146)
    \Edge[label=](8)(147)
    \Edge[label=](8)(63)
    \Edge[label=](9)(111)
    \Edge[label=](9)(147)
    \Edge[label=](9)(86)
    \Edge[label=](9)(127)
    \Edge[label=](10)(39)
    \Edge[label=](10)(109)
    \Edge[label=](10)(14)
    \Edge[label=](10)(112)
    \Edge[label=](10)(84)
    \Edge[label=](10)(27)
    \Edge[label=](11)(43)
    \Edge[label=](11)(60)
    \Edge[label=](12)(35)
    \Edge[label=](12)(133)
    \Edge[label=](12)(109)
    \Edge[label=](12)(45)
    \Edge[label=](12)(46)
    \Edge[label=](12)(47)
    \Edge[label=](12)(49)
    \Edge[label=](12)(114)
    \Edge[label=](12)(143)
    \Edge[label=](12)(28)
    \Edge[label=](12)(30)
    \Edge[label=](13)(34)
    \Edge[label=](13)(69)
    \Edge[label=](13)(72)
    \Edge[label=](13)(18)
    \Edge[label=](13)(20)
    \Edge[label=](14)(32)
    \Edge[label=](14)(35)
    \Edge[label=](14)(40)
    \Edge[label=](14)(64)
    \Edge[label=](14)(43)
    \Edge[label=](14)(44)
    \Edge[label=](14)(16)
    \Edge[label=](14)(140)
    \Edge[label=](14)(85)
    \Edge[label=](15)(66)
    \Edge[label=](15)(39)
    \Edge[label=](15)(51)
    \Edge[label=](15)(30)
    \Edge[label=](15)(31)
    \Edge[label=](16)(132)
    \Edge[label=](16)(102)
    \Edge[label=](16)(40)
    \Edge[label=](16)(44)
    \Edge[label=](16)(17)
    \Edge[label=](17)(48)
    \Edge[label=](17)(119)
    \Edge[label=](17)(140)
    \Edge[label=](17)(87)
    \Edge[label=](18)(70)
    \Edge[label=](18)(119)
    \Edge[label=](20)(104)
    \Edge[label=](20)(105)
    \Edge[label=](20)(75)
    \Edge[label=](20)(78)
    \Edge[label=](20)(143)
    \Edge[label=](20)(120)
    \Edge[label=](20)(29)
    \Edge[label=](21)(132)
    \Edge[label=](21)(139)
    \Edge[label=](21)(53)
    \Edge[label=](24)(115)
    \Edge[label=](25)(137)
    \Edge[label=](25)(26)
    \Edge[label=](26)(56)
    \Edge[label=](26)(55)
    \Edge[label=](26)(41)
    \Edge[label=](27)(69)
    \Edge[label=](27)(149)
    \Edge[label=](27)(54)
    \Edge[label=](27)(88)
    \Edge[label=](28)(32)
    \Edge[label=](30)(46)
    \Edge[label=](31)(90)
    \Edge[label=](32)(45)
    \Edge[label=](33)(76)
    \Edge[label=](35)(56)
    \Edge[label=](36)(65)
    \Edge[label=](36)(74)
    \Edge[label=](36)(113)
    \Edge[label=](37)(89)
    \Edge[label=](37)(135)
    \Edge[label=](37)(141)
    \Edge[label=](39)(144)
    \Edge[label=](39)(112)
    \Edge[label=](39)(52)
    \Edge[label=](39)(149)
    \Edge[label=](39)(54)
    \Edge[label=](39)(57)
    \Edge[label=](44)(108)
    \Edge[label=](45)(129)
    \Edge[label=](45)(67)
    \Edge[label=](48)(71)
    \Edge[label=](49)(88)
    \Edge[label=](50)(99)
    \Edge[label=](50)(148)
    \Edge[label=](50)(67)
    \Edge[label=](51)(80)
    \Edge[label=](51)(93)
    \Edge[label=](52)(96)
    \Edge[label=](52)(61)
    \Edge[label=](55)(131)
    \Edge[label=](55)(60)
    \Edge[label=](55)(59)
    \Edge[label=](55)(124)
    \Edge[label=](55)(62)
    \Edge[label=](56)(74)
    \Edge[label=](56)(58)
    \Edge[label=](56)(103)
    \Edge[label=](57)(131)
    \Edge[label=](59)(125)
    \Edge[label=](61)(110)
    \Edge[label=](61)(79)
    \Edge[label=](61)(81)
    \Edge[label=](61)(83)
    \Edge[label=](61)(84)
    \Edge[label=](63)(80)
    \Edge[label=](63)(136)
    \Edge[label=](63)(129)
    \Edge[label=](65)(83)
    \Edge[label=](67)(102)
    \Edge[label=](67)(144)
    \Edge[label=](67)(115)
    \Edge[label=](67)(92)
    \Edge[label=](69)(107)
    \Edge[label=](69)(122)
    \Edge[label=](70)(100)
    \Edge[label=](70)(101)
    \Edge[label=](70)(136)
    \Edge[label=](70)(126)
    \Edge[label=](73)(94)
    \Edge[label=](75)(128)
    \Edge[label=](75)(107)
    \Edge[label=](75)(82)
    \Edge[label=](75)(86)
    \Edge[label=](75)(125)
    \Edge[label=](77)(100)
    \Edge[label=](79)(97)
    \Edge[label=](79)(105)
    \Edge[label=](79)(95)
    \Edge[label=](80)(99)
    \Edge[label=](80)(98)
    \Edge[label=](81)(93)
    \Edge[label=](82)(127)
    \Edge[label=](84)(91)
    \Edge[label=](85)(120)
    \Edge[label=](87)(97)
    \Edge[label=](88)(137)
    \Edge[label=](89)(116)
    \Edge[label=](90)(142)
    \Edge[label=](95)(138)
    \Edge[label=](95)(116)
    \Edge[label=](99)(148)
    \Edge[label=](99)(106)
    \Edge[label=](101)(106)
    \Edge[label=](101)(114)
    \Edge[label=](102)(123)
    \Edge[label=](104)(146)
    \Edge[label=](108)(123)
    \Edge[label=](108)(117)
    \Edge[label=](109)(126)
    \Edge[label=](112)(121)
    \Edge[label=](124)(134)
    \Edge[label=](125)(130)
    \Edge[label=](128)(145)
\end{tikzpicture}
\label{dg}
\caption{Example Title}
\end{figure}


==> figures/visualizations/er/deep_walk_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/er/diffusion_ETT_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/er/diffusion_endpoint_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/er/node2vec_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/small/deep_walk_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/small/diffusion_ETT_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/small/diffusion_endpoint_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/small/node2vec_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/watts_2/deep_walk_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/watts_2/diffusion_ETT_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/watts_2/diffusion_endpoint_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]


==> figures/visualizations/watts_2/node2vec_2d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.4,transform shape]
\tikzstyle{VertexStyle}=[minimum size = 10pt,inner sep=0pt, shape = circle]

